Markov-Chain Monte-Carlo A Bayesian Approach to Statistical Mechanics

Since the middle of the 1940's scientists have used Monte Carlo (MC) simulations to obtain information about physical processes. This has proved a accurate and and reliable method to obtain this information. Through out resent years researchers has begone to use the slightly newer Markov Chain Monte Carlo (MCMC) simulation. This differs from the ordinary MC by using the Markov Chain. MCMC originates from Bayesian statistics. This method has given researchers a completely new tool to learn something about physical systems. One of the fields where MCMC is a good new tool, is astrophysics. Today MCMC is widely used in simulating power spectra for asteroseismic data. Hereby providing the scientists with important new information of stellar interiors. From our results we see that MCMC delivers a robust and reliable result with good error estimation. We also learn that MCMC is a power full tool which can be applied to a large verity of problems.

==> Montecarlo.tex <==
Since the 1940's scientist have been using Monte-Carlo (hence MC) for statistical modelling. MC or MC integration, as it is often called is a method used for obtaining knowledge about systems which are beyond the reach of analytical methods \cite {MC}.
Suppose that we randomly pick $N$ uniformly distributed points. in a multidimensional volume $V$. These points will be referred to as $x_{0}, ~x_{1}, ~\ldots , ~x_{N-1}$. Then we apply the underlying theorem of MC integration. 
\begin{equation}\label{eq:MCb}
	\int f dV \approx V \langle f \rangle \pm V \sqrt{\frac{\langle f^{2}\rangle-\langle f \rangle^{2}}{N}}
\end{equation} 
This theorem seen in \eqref{MCb} estimates the integra of the function $f$ over the multidimensional volume.  The angle brackets in \eqref{MCb} is simply the arithmetic mean ofer the $N$ sample points,
\begin{equation}\label{eq:MCf}
	\langle f\rangle \equiv \frac{1}{N}\sum_{i = 0}^{N-1}f(x_{i})\qquad\quad \langle f^{2} \rangle \equiv \frac{1}{N}\sum_{i = 0}^{N-1}f^{2}(x_{i})
\end{equation} 
One should notice the plus-minus sign in \eqref{MCb}, this is only an one standard deviation error estimate for the integral, not a rigorous bound. 

The MC approach have been used very extensively in the past, and through this approach we have learnt a lot, and it has proved itself, as a robust way of determine integrals numerically. So if this method is so good an robust why do we then need a new one? 

There are several reasons, first of all most MC simulations  uses only a pseudo-random sampling. Then depending on the random sampler one uses it will be determined whether or not it is a good estimate. Since it is dependant on the kind of random sampler one uses for the MC. 

==> histx_top0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5400.00,3780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1162,704){\makebox(0,0)[r]{\strut{} 5000}}%
      \put(1162,1407){\makebox(0,0)[r]{\strut{} 5500}}%
      \put(1162,2110){\makebox(0,0)[r]{\strut{} 6000}}%
      \put(1162,2813){\makebox(0,0)[r]{\strut{} 6500}}%
      \put(1162,3516){\makebox(0,0)[r]{\strut{} 7000}}%
      \put(1294,484){\makebox(0,0){\strut{} 2}}%
      \put(1645,484){\makebox(0,0){\strut{} 2.05}}%
      \put(1997,484){\makebox(0,0){\strut{} 2.1}}%
      \put(2348,484){\makebox(0,0){\strut{} 2.15}}%
      \put(2700,484){\makebox(0,0){\strut{} 2.2}}%
      \put(3051,484){\makebox(0,0){\strut{} 2.25}}%
      \put(3403,484){\makebox(0,0){\strut{} 2.3}}%
      \put(3754,484){\makebox(0,0){\strut{} 2.35}}%
      \put(4106,484){\makebox(0,0){\strut{} 2.4}}%
      \put(524,2110){\rotatebox{90}{\makebox(0,0){\strut{}$N$}}}%
      \put(2700,154){\makebox(0,0){\strut{}Slope $m$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{histx_top0}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> histy_top0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5400.00,3780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1162,704){\makebox(0,0)[r]{\strut{} 5000}}%
      \put(1162,1407){\makebox(0,0)[r]{\strut{} 5500}}%
      \put(1162,2110){\makebox(0,0)[r]{\strut{} 6000}}%
      \put(1162,2813){\makebox(0,0)[r]{\strut{} 6500}}%
      \put(1162,3516){\makebox(0,0)[r]{\strut{} 7000}}%
      \put(1294,484){\makebox(0,0){\strut{} 20}}%
      \put(1645,484){\makebox(0,0){\strut{} 25}}%
      \put(1997,484){\makebox(0,0){\strut{} 30}}%
      \put(2348,484){\makebox(0,0){\strut{} 35}}%
      \put(2700,484){\makebox(0,0){\strut{} 40}}%
      \put(3051,484){\makebox(0,0){\strut{} 45}}%
      \put(3403,484){\makebox(0,0){\strut{} 50}}%
      \put(3754,484){\makebox(0,0){\strut{} 55}}%
      \put(4106,484){\makebox(0,0){\strut{} 60}}%
      \put(524,2110){\rotatebox{90}{\makebox(0,0){\strut{}$N$}}}%
      \put(2700,154){\makebox(0,0){\strut{}$b$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{histy_top0}}%
    \gplfronttext
  \end{picture}%
\endgroup

